Quarantines as a Targeted Immunization Strategy

In the context of the recent COVID-19 outbreak, quarantine has been used to "flatten the curve" and slow the spread of the disease. In this paper, we show that this is not the only benefit of quarantine for the mitigation of an SIR epidemic spreading on a graph. Indeed, human contact networks exhibit a powerlaw structure, which means immunizing nodes at random is extremely ineffective at slowing the epidemic, while immunizing high-degree nodes can efficiently guarantee herd immunity. We theoretically prove that if quarantines are declared at the right moment, high-degree nodes are disproportionately in the Removed state, which is a form of targeted immunization. Even if quarantines are declared too early, subsequent waves of infection spread slower than the first waves. This leads us to propose an opening and closing strategy aiming at immunizing the graph while infecting the minimum number of individuals, guaranteeing the population is now robust to future infections. To the best of our knowledge, this is the only strategy that guarantees herd immunity without requiring vaccines. We extensively verify our results on simulated and real-life networks.

==> files/1quarantine-v1.tex <==
\section{One quarantine}
In this section, we study the effect of one quarantine on the structure of the graph. We are particularly interested in whether it is possible to achieve herd immunity, and how to minimize the total number of people who have been touched by the epidemic. For the remainder of the paper, we study perfect quarantines, as defined below:

\begin{definition}[Quarantine]
	We call quarantine the complete halt of the spread of the epidemic. During a quarantine, all infected nodes transition to the removed state, and no new nodes become infected.
\end{definition}

\subsection{The quarantine operator}
\begin{lemma}
	Let $u(t)$ be the fraction of nodes of degree 1 that are susceptible after letting the epidemic spread for time $t$. Suppose we declare a quarantine when $u(t)$ reaches the value $u$. Let $T_Q: \mathbb{N}^N \rightarrow \mathbb{R}^N$ be the operator representing the transformation of the  expected number of susceptible nodes after one iteration of letting the epidemic grow, then declaring a quarantine.   Then:
	
	$$ T_Q(\{P_k\}_{k=0}^{N-1}) = \{P_k \cdot u^k\}_{k=0}^{N-1}.$$
	\proof This is a direct implication of Lemma \ref{lem:highDegreeU} from the Preliminaries.
\end{lemma}

As it turns out, the number of nodes in the removed state can be computed easily from the above result.

\begin{claim}
	Let $g_0(z)$ be the generative function of the distribution of degrees. The expected fraction of nodes in the removed state after one quarantine $R_Q$ is:
	
	$$ R_Q = 1 - g_0(u).$$
	
	\proof Let $p_k$ be the fraction of nodes of degrees $k$ in the graph, so that $P_k = N\cdot p_k$. Notice that for $k\geq N$, there exist no nodes of that degree, so $p_k = 0$. The generative function of the distribution of degrees is $\displaystyle g_0(z) = \sum_{j=0}^{\infty} p_j z^j$. 
	\begin{align*}
	R_Q &= \frac{1}{N} \left(N - \sum_{j=0}^{N} T_Q(\{P_k\}_{k=0}^{N})_j \right) \\
	&= \frac{1}{N} \left(N  -  \sum_{j=0}^{N} P_j \cdot u^j \right) \\
	 &= 1 -  \sum_{j=0}^{\infty} p_j \cdot u^j \\
	&= 1 - g_0(u).
	\end{align*}
\end{claim}

\subsection{Achieving herd immunity}
\subsubsection{General graphs}


We first establish  results for general graphs:

\begin{claim}
	Let $u$ be the remaining fraction of susceptible nodes of degree 1 when we start the quarantine. We achieve herd immunity for $u$ such that:
	$$ u^2 g_0''(u) - u g_0'(u) \leq 0.$$
	\proof Following Claim \ref{cl:herdImmunity}, we want to find $u$ such that $\E_{T_Q}[k^2] - 2 \E_{T_Q}[k] \leq 0$. This translates to:
	\begin{align*}
	\E_{T_Q}[k^2] - 2 \E_{T_Q}[k] &= \sum_{k=0}^{\infty} P_k \cdot u^{k} k^2 - 2 \sum_{k=0}^{\infty} P_k \cdot u^{k} k \\
	&= \sum_{k=0}^{\infty} P_k \cdot u^{k} k^2 -  \sum_{k=0}^{\infty} P_k \cdot u^{k} k -  \sum_{k=0}^{\infty} P_k \cdot u^{k} k \\
	&= \sum_{k=0}^{\infty} P_k \cdot u^{k} k(k-1)  - \sum_{k=0}^{\infty} P_k \cdot u^{k} k \\
	&= u^2 g_0''(u) - u g_0'(u)\\
	&\leq 0.
	\end{align*}
\end{claim}

\subsubsection{Powerlaw graphs}
We give some numerical results for powerlaw graphs:
\begin{claim} \label{cl:u}
	Let $u$ be the remaining fraction of susceptible nodes of degree 1 when we start the quarantine. For an infinite powerlaw graph of exponent 3, we achieve herd immunity for $u \leq 0.940599$.
	\proof We want to find $u$ such that:
	\begin{align*}
	\E_{T_Q}[k^2] - 2 \E_{T_Q}[k] 
	&= \sum_{k=1}^{\infty} \frac{C}{k^3} \cdot u^{k} k^2 - 2 \sum_{k=1}^{\infty} \frac{C}{k^3} \cdot u^{k} k \\
	&= C \sum_{k=1}^{\infty} \frac{u^{k}}{k}   - 2  \frac{u^{k}}{k^2} \\
	&= -C \cdot \left(2 Li_2(u) - \log(1-u) \right)\\
	&\leq 0.
	\end{align*}
	Where $Li_2(u)$ is the polylog-2 function. Solving this equation numerically yields $u \leq 0.940599$.
\end{claim}

We now look at the total number of nodes in the removed state in this case:

\begin{claim} \label{cl:rq}
	If we declare a quarantine when a fraction $u' = 0.940599$ of nodes of degree 1 are still in the susceptible state, then by the end of quarantine, at least $R_Q = 92.2912\%$ of the nodes are still in the susceptible state.
	\proof Remembering that $C = \frac{1}{\zeta(3)}$, where $\zeta(x) = \sum_{k=1}^{\infty} \frac{1}{k^x}$, the number of susceptible nodes is: 
	$$g_0(u') \geq \displaystyle\frac{1}{\zeta(3)}\sum_{k=1}^N \frac{u'^k}{k^3} \approx 0.922912. $$
\end{claim}

Combining Claims \ref{cl:u} and \ref{cl:rq}, the network can therefore achieve herd immunity while infecting a bit less than $8\%$ of the nodes:

\begin{theorem}
	For powerlaw graphs of exponent 3, min-degree 1, it is possible to achieve herd immunity by declaring a single quarantine when a bit less than $6\%$ of the nodes of degree 1 are infected. In this case, less than $8\%$ of the nodes will be removed at the end of the quarantine.
\end{theorem}

\underline{Remarks:} 
\begin{itemize}
	\item  Quarantines can have extremely positive side effects, including achieving herd immunity.
	\item  When herd immunity is achieved, there exists an epidemic threshold, and measures to slow the spread ($e.g.$ washing hands) become impactful. 
	\item  The result above is both positive (only $8\%$ of removed nodes) and disappointing: this is the best achievable, in the sense that nothing else we can do in this optimistic quarantine model can reduce the fraction of removed nodes at the end. In most cases, $8\%$ of the population being infected represents millions of people, and is not desirable.
	\item  Having reached herd immunity does not mean that the disease dies out, but rather that only a fraction of the graph will be infected. What we might desire instead is to minimize the total number of removed nodes at the end, if the epidemic started again after the quarantine. 
\end{itemize} 

We study this last point experimentally in section \ref{sec:exp}.

\begin{comment}
\subsection{Minimizing the final number of removed nodes}
\subsubsection{General graphs}
Even when we have reached herd immunity, a large fraction of the population ca still become infected. Indeed, the expected total number of nodes in the removed state at the end of an epidemic is given by:

\begin{claim}[From Newman \cite{}]\label{cl:S}
	Let $\phi$ be the probability that an infected node infects its susceptible neighbor, and $g_0$ be the generative function of the degrees of the nodes in the graph, and $g_1$ the generative function of the excess degrees. Then the expected number of removed nodes at the end of the epidemic $S$ is given by:
	$$ S= 1 - g_0(v),$$
	where $v$ is the solution of the equation:
	$$ v = 1 - \phi + \phi g_1(v).$$
	\proof See Newman.
\end{claim}

We can compute the generative functions of the degrees and the excess degrees of the graph after a quarantine has been declared:

\begin{claim}\label{cl:g0Q}
	Let $g_0^Q$ and $g_1^Q$ be the generative functions of the degrees and the excess degrees of the resulting graph after a quarantine has been declared when a fraction $u$ of the nodes of degree 1 remain susceptible. Then:
	\begin{align*}
	g_0^Q(z) &= \frac{g_0(u\cdot z)}{g_0(u)} \\
	g_1^Q(z) &= \frac{g_1(u\cdot z)}{g_1(u)}.
	\end{align*}
	\proof Let $p_k^Q$ and $q_k^Q$ be the distribution of degrees and excess degrees after a quarantine. Using Claim \ref{lem:highDegreeU}, we know $p_k^Q = \frac{u^k \cdot p_k}{g_0(u)}$. Then:
	\begin{align*}
	g_0^Q(z) &= \sum_{k=0}^{\infty} p_k^Q z^k \\
	&= \frac{1}{g_0(u)}\sum_{k=0}^{\infty} p_k \cdot (u \cdot z)^k \\
	&= \frac{g_0(u\cdot z)}{g_0(u)}.
	\end{align*}
	Similarly, since $g_1(z) = \frac{g_0'(z)}{g_0'(1)}$, we have:
%	\begin{align*}
%	g_1^Q(z) &= \frac{g_0^Q'(z)}{g_0'(1)} \\
%	&= \sum_{k=0}^{\infty} \frac{(k+1)p_{k+1}^Q}{<k>} z^k \\
%	&= \frac{1}{g_0(u)}\sum_{k=0}^{\infty} \frac{(k+1)p_{k+1} u^{k+1}}{<k>} z^k \\
%	&= u\frac{u}{g_0(u)} \cdot \sum_{k=0}^{\infty} q_k \cdot  (u \cdot z)^k \\
%	&= \frac{u\cdot g_1(u\cdot z)}{g_0(u)}.
%	\end{align*}
%	
	\begin{align*}
	g_1^Q(z) &= \frac{g_0^{'Q} (z)}{g_0^{'Q} (1)} \\
	&= \frac{u\frac{g_0'(u\cdot z)}{g_0(u)}}{u\frac{g'_0(u\cdot 1)}{g_0(u)}} \\
	&= \frac{g'_0(1)}{g'_0(1)} \cdot \frac{g_0'(u\cdot z)}{g'_0(u)} \\
	&= \frac{g_1(u\cdot z)}{g_1(u)}.
	\end{align*}
\end{claim}

Now, it is possible to express the total number of removed nodes $R$ as a function of $u$, the fraction of susceptible nodes when we declare the quarantine:
\begin{lemma}
	Suppose we declare a quarantine when a fraction $u$ of nodes of degree 1 remain susceptible, then have an outbreak start again after the quarantine. The total expected fraction of removed nodes $R(u)$ is given by:
	$$ R(u) = 2 - g_0(u) -  \frac{g_0(u\cdot v)}{g_0(u)},$$
	with$v$ solution of $ v  = 1 - \phi + \phi \frac{ g_1(u\cdot z)}{g_1(u)}$.
	\proof 
	Let $R^Q(u)$ be the number of removed nodes at the end of a quarantine, and $S^Q(u)$ be the expected number of removed nodes if an outbreak starts again after the quarantine. The total expected fraction of removed nodes is given by $R(u) = R^Q(u) + S^Q(u)$.
	We know, according to Claim \ref{cl:rq}, that: 
	$$R^Q(u) = 1 - g_0(u).$$ 
	According to Claims \ref{cl:S} and \ref{cl:g0Q}, we also have:
	$$S^Q(u) = 1 - g_0^Q(v) = 1 - \frac{g_0(u\cdot v)}{g_0(u)},$$
	with $v$ solution of $ v = 1 - \phi + \phi g_1^Q(v) = 1 - \phi + \phi \frac{g_1(u\cdot v)}{g_1(u)}$, which conclude the proof.
\end{lemma}

The equations above do not have close form solutions in general. For powerlaw graph, such a close form solution does not exist either. However, we can provide numerical approximations. 

\subsubsection{Applications to powerlaw graphs}
Using parameters for COVID-19 from [cite], let us assume $\phi = 1 - e^{-\beta \cdot \tau}$, with $\beta = 0.2$, and $\tau= 10$. Then, $\phi = 1 - e^{-2}$.

\begin{claim}
	Let us consider an infinite powerlaw graph of parameter $\alpha=3$ Suppose we declare a quarantine when a fraction $u$ of nodes of degree 1 remain susceptible, then have an outbreak start again after the quarantine. The total expected fraction of removed nodes $R(u)$ is given by:
	$$ R(u) = 2 - \frac{Li_3(u)}{\zeta(3)} - \frac{Li_3(u \cdot v)}{Li_3(u)},$$
	with $v$ solution of $ v = e^{-2}+ (1-e^{-2}) \cdot \frac{Li_2(u \cdot v)}{v \cdot Li_2(u)}$.
	\proof \begin{align*}
	g_1^Q(z) &= \frac{g_1(u\cdot z)}{g_1(u)} \\
	&= \frac{\frac{Li_2(uz)}{uz \zeta(2)}}{\frac{Li_2(u)}{u \zeta(2)}} \\
	&= \frac{Li_2(uz)}{z Li_2(u)}.
	\end{align*}
\end{claim}

\begin{lemma}
	The best total expected number of removed nodes $R_{min}$ is:
	$$ R_{min} = .$$
	It is achieved if we declare a quarantine when $u = $.
	\proof 
	Let $R^Q(u)$ be the number of removed nodes at the end of a quarantine, and $S^Q(u)$ be the expected number of removed nodes if an outbreak starts again after the quarantine. The total expected number of removed nodes is given by $R(u) = R^Q(u) + S^Q(u)$.
	We know, according to Claim \ref{cl:rq}, that: 
	$$R^Q(u) = 1 - g_0(u).$$ 
	According to Claims \ref{cl:S} and \ref{cl:g0Q}, we also have:
	$$S^Q(u) = 1 - g_0^Q(f(u)) = 1 - g_0(u\cdot f(u)),$$
	with $f(u)$ solution of $ f(u) = 1 - \phi + \phi g_1^Q(f(u)) = 1 - \phi + \phi \cdot u \cdot g_1(u\cdot f(u))$.
\end{lemma}


\subsection{Maximum number of infected nodes}
The maximum number of infected nodes during this process is {\color{red} FILL}. In practice, for a city of size $N=$, this is higher than the number of beds we can expect in hospitals [cite]. We know turn to another quarantine strategy which allows multiple smaller quarantines.
\end{comment}

==> files/old_experiments.tex <==
% EXPERIMENT SECTION OUTLINE:
% 1) Setup and introduction 
% 2) Results with a single quarantine on BA graphs 
% 3) Results on graphs with community structure / COVID parameters 
% 4) Results when multiple quarantines are considered
% 5) Results when spreading model is modified 
% 6) Discussion + Experiment conclusion 

\section{Experiments}\label{sec:exp}

In this section, we validate the theoretical results described above by simulating the course of an SIR epidemic with perfect quarantines on randomly generated and real networks. Simulations were run using a continuous-time event-driven algorithm \cite{Miller2019}. An infection is initialized by uniformly randomly selecting $\rho$ nodes to be infected.  We simulate perfect quarantines by moving all nodes in the I compartment to the R compartment and uniformly randomly selecting $\rho$ susceptible nodes to become infected after quarantine. All simulations are run until there are no more infected nodes. 

\subsection{Single Quarantine on Barabási-Albert Graphs} 
The first series of experiments focuses on the well-studied Barabási-Albert (BA) class of random graphs. BA graphs are scale-free, with a degree distribution that falls off according to the cubic powerlaw: $P(k)\sim k^{-3}$. For this first set of experiments, we consider a BA graph with 10K nodes, with parameter $m=5$. We will initially consider an infection with spreading and recovery rates equal, both set to $0.1$, and we set the number of infected nodes post-quarantine, $\rho$, to be 10. We find that the results we will present are fairly insensitive to the choice of graph parameters or infection parameters.

We consider the effect of performing a single quarantine, which is triggered once a fixed proportion of the population is either infected or recovered, a quantity which we denote the quarantine threshold. We consider quarantine thresholds ranging from $0$ to $1$, with increments of $0.01$, and run 100 trials for each fixed threshold. 


%%%%% FIRST FIGURE: SINGLE Q I/R PLOTS 


\begin{figure}[H]%
	\centering
	\begin{subfigure}{.45\linewidth}
		\includegraphics[width=\textwidth]{figures/ba_singleQ_I_cleaner.png}
		\caption{Infected nodes by time on a BA graph with a single quarantine.}
	\end{subfigure}
	\hskip2em
	\begin{subfigure}{.45\linewidth}
		\includegraphics[width=\textwidth]{figures/ba_singleQ_R_cleaner.png}
		\caption{Recovered nodes by time on a BA graph with a single quarantine.}
	\end{subfigure}
	\caption{Simulations run on a BA graph with 100K nodes. The blue curve indicates no quarantine, the red curve demonstrates the single-quarantine strategy that minimizes the final number of recovered nodes, and the green curve demonstrates the single-quarantine strategy that minimizes the maximum number of infected nodes.}
	\label{fig:ba-single-IR}%
\end{figure}

The two criteria we will examine are the final number of recovered nodes and the maximum number of infected nodes. The final number of recovered nodes indicates how many nodes will have become infected throughout the course of the epidemic. The maximum number of infected nodes was shown to be an important quantity of interest during the COVID-19 pandemic, as hospitals operating above their capacity were forced to make tragic choices between patients in need of treatment. Figure \ref{fig:ba-single-IR} demonstrates the single-quarantine strategies that minimize either of these two criteria. Qualitatively, the minimum of the maximum number of infected nodes will be attained by enacting a quarantine that roughly balances the number of infected nodes at quarantine-time with the peak that is attained after quarantine. However, to minimize the final number of recovered nodes, a quarantine should be enacted just before the epidemic peaks, to effectively neutralize the second wave of the infection. Here we notice that the optimal single-quarantine strategy differs depending on which criterion we seek to minimize. We examine this further in figure \ref{fig:ba-single-optima}(a) where we plot these two quantities versus the quarantine threshold. We observe that each of these quantities exhibits a V-like curve, however their minima are attained at different quarantine thresholds. 



\begin{figure}[H]%
    \centering
        \begin{subfigure}{.48\linewidth}
    	\includegraphics[width=\textwidth]{figures/ba_singleQ_props_cleaner.png}
    	\caption{Maximum number of infected individuals and final number of recovered individuals plotted versus quarantine threshold. Notice that the y-axes differ. There is a clear optimal quarantine threshold depending on the objective, however these optima do not align.}
    \end{subfigure}
    \hskip2em
    \begin{subfigure}{.43\linewidth}
    \includegraphics[width=\textwidth]{figures/ba_singleQ_R_hist.png}
    	\caption{Final number of recovered nodes when quarantines are enacted near the optimal quarantine threshold. Observe that as the quarantine threshold approaches the optimum, the number of outbreaks decreases, as does the extent of each outbreak.}
    \end{subfigure}
    \caption{Examining single-quarantine strategies}
    \label{fig:ba-single-optima}%
\end{figure}




As alluded to by our theory, a perfect quarantine serves as an organic form of targeted immunization and favors the removal of high-degree nodes, yielding a graph in the configuration model with a lighter-tailed degree distribution. We conjecture that this has a twofold effect in reducing the final number of infected nodes. Primarily, the graph structure is broken up enough to reduce the number of nodes that become infected in the event that an outbreak does occur; and secondarily, the probability of an outbreak occurring decreases after a reinitialization of the infection post-quarantine. This effect is demonstrated in figure \ref{fig:ba-single-optima}(b) where we plot a histogram of the final number of recovered nodes on multiple simulations for multiple runs with a fixed quarantine threshold. The bimodal distribution indicates that many reinitializations peter out quickly and outbreaks do not occur. However, some outbreaks do occur, but yield smaller numbers of final-recovered nodes than a no-quarantine scenario. 

When the quarantine is declared at the optimal moment, there is no significant new outbreak after the quarantine is over, as can be seen by the flat red curve in Figure \ref{fig:ba-single-IR}(b). This is despite infecting a fraction $\rho$ of the population: with this simple quarantine, the new network is now robust to future outbreaks. Quarantining therefore constitutes a valid immunization strategy.

\subsection{Two Quarantines on Barabási-Albert Graphs}
\begin{figure}[H]%
	\centering
	\begin{subfigure}{.45\linewidth}
		\includegraphics[width=\textwidth]{figures/ba_doubleQ_I_cleaner.png}
		\caption{Infected nodes by time on a BA graph with two quarantines.}
	\end{subfigure}
	\hskip2em
	\begin{subfigure}{.45\linewidth}
		\includegraphics[width=\textwidth]{figures/ba_doubleQ_R_cleaner.png}
		\caption{Recovered nodes by time on a BA graph with two quarantines.}
	\end{subfigure}
 \caption{Simulations run on a BA graph with 100K nodes. The blue curve indicates no quarantine, the red curve demonstrates the double-quarantine strategy that minimizes the final number of recovered nodes, and the green curve demonstrates the double-quarantine strategy that minimizes the maximum number of infected nodes.}%
\label{fig:ba-double-IR}%
\end{figure}



Now we consider the effect of running two quarantines on a BA graph. The graph settings as well as the epidemic parameters and reinitialization model are kept the same from the single-quarantine section. We enact two perfect quarantines at thresholds $Q_1, Q_2$, where the first quarantine is enacted when $Q_1$ fraction of the population is either infected or recovered, and the second quarantine is enacted when $Q_2$ proportion of the total population has entered either the infected or recovered compartments \emph{after the first quarantine}. We perform a grid search over values of $Q_1, Q_2$ and report the maximum number of infected nodes as well as the final number of recovered nodes in Figure \ref{fig:ba-double-heatmap}. The number of infected and recovered nodes for the quarantine settings that attain optimal criteria are plotted against the no-quarantine scenario in Figure \ref{fig:ba-double-IR}.


\begin{figure}[H]%
	\centering
	\begin{subfigure}{.45\linewidth}
		\includegraphics[width=\textwidth]{figures/ba_doubleQ_heatmap_R.png}
		\caption{Final recovered nodes with two quarantines. Darker means fewer nodes were infected.}
	\end{subfigure}
	\hskip2em
	\begin{subfigure}{.45\linewidth}
		\includegraphics[width=\textwidth]{figures/ba_doubleQ_heatmap_I.png}
		\caption{Maximum number of infected nodes with two quarantines. Lighter colors correspond to smaller peaks.}
	\end{subfigure}
	\caption{Heatmaps displaying the final recovered nodes and maximum infected nodes under various two-quarantine strategies. Observe that two quarantines cannot achieve a noticeably lower number of final recovered nodes, and the optimum is attained when the sum of $Q1$ and $Q2$ is equivalent to the optimal quarantine threshold in the single-quarantine setting. The maximum number of infected nodes is displayed on the right: notice that the optimal two-quarantine strategy here has both quarantines occur earlier than the optimal strategy for minimizing R.}%
	\label{fig:ba-double-heatmap}%
\end{figure}




Examining the heatmap in Figure \ref{fig:ba-double-heatmap}(a) that displays the final number of recovered nodes in a two-quarantine setting, we observe the following qualitative trends. The dark-colored bands indicate quarantine strategies that have low numbers of final recovered nodes, which are most prevalent along a horizontal line and a diagonal line, i.e. the set of gridpoints such that $Q_1+Q_2$ is fixed at 0.64, which is the optimal value for the single quarantine setting. This indicates that there is not much benefit to enacting a second quarantine, if the first quarantine was enacted at the correct time. 

The heatmap in Figure \ref{fig:ba-double-heatmap}(b) displays the maximum number of infected nodes. The lighter patches indicate lower maximum numbers of infected nodes, and can qualitatively be characterized as a triangular patch bordered on the bottom by a horizontal band. The horizontal banding is indicative of the first peak dominating, whereas the light triangular patch represents the regime where the quarantines are enacted to roughly balance the height of all three peaks. One should also observe that both the minimal horizontal band and the minimal triangular patch in the right heatmap are higher and shifted to the left from the minimal bands in the left heatmap. This supports the trend observed in the single quarantine setting that quarantines should be enacted earlier to minimize maximal number of individuals infected at any one point, whereas quarantines should be enacted later to minimize the total number of infected individuals. 
 
\subsection{Multiple quarantines}
As discussed before, minimizing the maximum number of infected nodes or the total number of removed nodes happens for different quarantine thresholds. In this section, we want to achieve the best of both worlds: minimizing the total number of removed nodes while never letting the maximum number of infected nodes rise above a certain threshold.

This is achieved in a slightly different setting than before. Instead of declaring a quarantine when a certain threshold is reached, we declare it when a certain value of infected nodes is reached. The results are below:

\begin{figure}[H]%
	\centering
		\includegraphics[width=0.6\textwidth]{figures/many-quarantines.png}
		\caption{Final fraction of recovered nodes with as many quarantines as needed, as a function of the number of infected nodes when we declare the quarantine.}
	\label{fig:many-quarantines}%
\end{figure}

Our first observation is that there exist some quarantine strategies which allow for about $65\%$ of removed nodes, which is the optimal final number of removed nodes in the case of a single quarantine. We also notice that many of these strategies exist, which would allow for an adapted strategy depending on the size of the city in which it's deployed. Finally, although some strategies perform much worse than others, they all are an improvement compared to never deploying a quarantine.

